Streaming Heteroscedastic Probabilistic PCA with Missing Data

Streaming principal component analysis (PCA) is an integral tool in large-scale machine learning for rapidly estimating low-dimensional subspaces from very high-dimensional data arriving at a high rate. However, modern datasets increasingly combine data from a variety of sources, and thus may exhibit heterogeneous quality across samples. Standard streaming PCA algorithms do not account for non-uniform noise, so their subspace estimates can quickly degrade. While the recently proposed Heteroscedastic Probabilistic PCA Technique (HePPCAT) addresses this heterogeneity, it was not designed to handle streaming data, which may exhibit non-stationary behavior. Moreover, HePPCAT does not allow for missing entries in the data, which can be common in streaming data. This paper proposes the Streaming HeteroscedASTic Algorithm for PCA (SHASTA-PCA) to bridge this divide. SHASTA-PCA employs a stochastic alternating expectation maximization approach that jointly learns the low-rank latent factors and the unknown noise variances from streaming data that may have missing entries and heteroscedastic noise, all while maintaining a low memory and computational footprint. Numerical experiments demonstrate the superior subspace estimation of our method compared to state-of-the-art streaming PCA algorithms in the heteroscedastic setting. Finally, we illustrate SHASTA-PCA applied to highly heterogeneous real data from astronomy.

==> s,intro.tex <==
% !TEX root = main.tex
% s,intro

\section{Introduction}
\label{sec:intro}

Modern data are increasingly large in scale
and formed by combining heterogeneous samples from diverse sources or conditions
and exhibit heteroscedastic noise, or noises of different variances \citep{hong2021heppcat}.
For example, in environmental monitoring,
data from a few high-precision instruments
may be combined with a large volume of less precise crowd-sourced data~\citep{hong2021heppcat}.
In astronomy, quasar spectra vary widely in quality across samples \citep{ahumada202016th}.
Recent advances in machine learning also consider data of heterogeneous quality,
where data from different sources of varying quality
are combined to leverage additional training samples.
Many examples of this occur in settings such as medical imaging;
MRI coils exhibit varying signal-to-noise ratios \citep{pruessmann1999sense},
and computed tomography images vary in quality by radiation dose
\citep{anam2020CTmeanfilter}. 
% \textcolor{red}{[citation?]}

Principal component analysis (PCA) for visualization, exploratory data analysis,
data compression, predictive tasks, or other downstream tasks
is one of the most fundamental tools in machine learning.
\tmlrrev{PCA and factor analysis are especially important to applications with heterogenous noise, such as in cryo-electron microscopy images \citep{anden2017factor, bendory2020single}.}
Well-studied and computable via a singular value decomposition or eigendecomposition, PCA requires a fully observed batch of data to estimate the batch's principal components. However, in many applications, due to memory or physical constraints, the full data cannot be observed in its entirety at computation time and is instead read partially into memory piece by piece, or observations may stream in continuously and indefinitely.
Likewise, the signal may evolve over time and require adaptive tracking algorithms for the low-rank component. Adding to these difficulties, it is also common for big data to contain missing entries. Magnetic resonance imaging (MRI) scans may subsample spatial frequencies \citep{mensch2017stochastic}, most user ratings of titles in collaborative filtering datasets are unobserved \citep{candesplan2010matrixcompletion}, and environmental sensing readings may occasionally drop out \citep{sensor_network_data_fault_types2009}. Consequently, there is a need for PCA techniques that can handle heteroscedastic noise, missing data, and scalability issues.

A tremendous body of work has studied streaming PCA techniques for learning a signal subspace from noisy incremental data observations with missing entries. Streaming or online PCA algorithms often enjoy the advantages of computational efficiency, low memory overhead, and adaptive tracking abilities, making them very useful in real world big data applications.
However, no existing streaming methods account for noise with different variances across samples, i.e., samplewise heteroscedastic noise, and their estimates can be highly corrupted by the noisiest samples. The work in~\citet{hong2021heppcat} developed a Heteroscedastic Probabilistic PCA technique (HePPCAT) for data with varying noise levels across samples.
HePPCAT learns the low-rank factors and the unknown noise variances via maximum likelihood estimation, but only in the batch setting with fully observed entries. Other batch heteroscedastic PCA algorithms, like weighted PCA studied in \citet{jolliffe2002pca, young1941mle, hong2023owp} and HeteroPCA \citep{zhang:18:hpa} for data with heteroscedastic features, also lack streaming and adaptive tracking abilities.
\tmlrrev{With no existing methods capable of handling missing entries, heteroscdastic noise, and streaming data, this non-trivial task requires deriving new algorithms.
}

To the best of our knowledge, this paper is the first work to develop a streaming PCA algorithm for data with missing entries and heteroscedastic noise.
Our algorithm jointly estimates the factors and unknown noise variances in an \emph{online} fashion from streaming incomplete data using an alternating stochastic minorize-maximize (SMM) approach with small computational and memory overhead.
\tmlrrev{
We carefully and precisely derive the minorizers and design a particular alternating schedule of stochastic updates that distinguishes our approach from existing SMM methods. Notably, we show that missing entries and heteroscedastic noise require more complex updates, unlike the simpler algebraic formulations computed in algorithms like HePPCAT or PETRELS \citep{chi_petrels2013}.
}
We demonstrate that our algorithm can achieve better estimation of the signal subspace (without knowledge of the noise variances) from subsampled data compared to state-of-the-art streaming PCA methods that assume homogeneous noise.
Our algorithm \tmlrrev{is unique in that it} not only tracks low-dimensional dynamic subspaces, but can also track dynamic noise variances that occur in applications related to sensor calibration \citep{jun2003drift} \tmlrrev{and beamforming in nonstationary noise environments \cite{cohen2004nonstationary}}. 
\tmlrrev{Finally, this work extends our understanding of streaming PCA to the setting with heteroscedastic noise and draws connections to existing work in the literature. 
In particular, the proposed method closely relates to the streaming PCA algorithm PETRELS \citep{chi_petrels2013}, but differs by learning the noise variances of the data on-the-fly and downweighting noisier data samples in the factor updates.
Furthermore, we show that our proposed method implicitly optimizes a regularized least-squares problem whose adaptive hyperparameter varies by the learned heterogeneous noise variances.}

\Cref{shasta:sec:rel} discusses related works for both streaming PCA and heteteroscedastic PCA.
\Cref{sec:sppca} describes the model we consider, the resulting optimization problem, and the proposed algorithm. \Cref{sec:results} presents synthetic and real data experiments that demonstrate the benefits of the proposed method over existing state-of-the-art streaming PCA algorithms. 

\subsection{Notation}

We use bold upper case letters $\bmA$ to denote matrices, bold lower case letters $\bmv$ to denote vectors, and non-bold lower case letters $c$ for scalars. We denote the Hermitian transpose of a matrix as $\bmA'$ and the trace of a matrix as $\tr(\bmA)$.
% The spectral norm of a matrix is denoted by $\|\bmA\|$ and the Frobenius norm by \normfrob{\bmA}.
The Euclidean norm is denoted by $\|\cdot\|_2$.
The identity matrix of size $d$ is denoted as $\bmI_d$. The notation $i \in [k]$ means $i=1,\dots,k$.



==> test-alg,shasta2.tex <==
\subsection{SHASTA-PCA-2}

Our algorithm uses a stochastic EM approach to maximize the empirical loss function over the streamed samples. Using a sequence of weights $(w_t)_{t\geq1}$, where $w_t \in (0,1)$, and trust-region parameters $c_F, c_v > 0$, we construct an approximate minorizer $\bbrPsi_t(\bmF,\bmv)$ using aggregated past information and perform block-coordinate maximization of $\bbrPsi_t(\bmF,\bmv)$ between the blocks $\bmF$ and $\bmv$. To summarize, the algorithm performs
\begin{align}
    \bbrPsi_t(\bmF,\bmv) &\leftarrow (1-w_t)\bbrPsi_{t-1}(\bmF,\bmv) + w_t \Psi_t(\bmF,\bmv; \bmF_t,\bmv_t) \nonumber \\
    \bmF_{t+1} &= \argmax_{\bmF:~\|\bmF - \bmF_t\|_2 \leq c_F w_t} \bbrPsi_t(\bmF,\bmv_t) \\
    \bmv_{t+1} &= \argmax_{\bmv:~ \|\bmv - \bmv_t\|_2 \leq c_v w_t} \bbrPsi_t(\bmF_{t+1},\bmv) \nonumber
\end{align}

Updating $\bbrPsi_t(\bmF,\bmv)$ proceeds as follows:
\begin{align}
    \bbrPsi_t(\bmF,\bmv) &= \sum_{\ell=1}^L -\bar{\theta}_{t,\ell} \log(v_\ell) - \frac{1}{v_\ell}(\bar{\alpha}_{t,\ell} - 2\bar{\rho}_{t,\ell}(\bmF)) \label{eq:joint_minorizer_Fv}\\
    \bar{\theta}_{t,\ell} &= (1-w_t)\bar{\theta}_{t-1,\ell} + w_t \mathbf{1}(\ell)  |\Omega_t| \\
    \bar{\alpha}_{t,\ell} &= (1-w_t)\bar{\alpha}_{t-1,\ell} + w_t \mathbf{1}(\ell) \|\bmy_{\Omega_t}\|_2^2 \\
    \bar{\rho}_{t,\ell}(\bmF) &= \sum_{i=1}^d \bmf_i' \bbrs_{t,\ell}(i) - \frac{1}{2} \bmf_i' \bbrR_{t,\ell}(i) \bmf_i \label{eq:shasta2:rhob}\\
     \bbrs_{t,\ell}(i) &= (1-w_t) \bbrs_{t-1,\ell}(i) + w_t \mathbf{1}(\ell) \bms_{t,\ell}(i) \\
    \bbrR_{t,\ell}(i) &= (1-w_t) \bbrR_{t-1,\ell}(i) + w_t \mathbf{1}(\ell)\bmR_{t,\ell}(i)\\
    \bms_{t,\ell}(i) &= \Omega_t(i) y_t(i) \bbrz_{t,\ell} \\
    \bmR_{t,\ell}(i) &= \Omega_t(i) (\bbrz_{t,\ell} \bbrz_{t,\ell}' + v_{t,\ell} \bar{\bmM}_{t,\ell})
\end{align}

\subsubsection{Optimizing \texorpdfstring{$\bmF$}{F}
  for fixed \texorpdfstring{$\bmv$}{v}}
  
 Holding $\bmv$ fixed as $\bmv_t$, optimizing \cref{eq:joint_minorizer_Fv} with respect to $\bmF$ can be expressed as $d$ separable quadratics in the rows of $\bmF$ for $i \in [d]$. For $i \in \Omega_t$, these quadratics have the following solutions
 \begin{align}
     \hat{\bmf}_i &= \left(\sum_{\ell=1}^L \frac{1}{v_{t,\ell}} \bbrR_{t,\ell}(i)\right)^{-1} \left(\sum_{\ell=1}^L \frac{1}{v_{t,\ell}} \bbrs_{t,\ell}(i)\right)
 \end{align}
 that can be computed in parallel, with no updates occurring for the rows $i \notin \Omega_t$. Then we take a step in the trust region, computing $\bmF_{t+1} = (1-c_F w_t) \bmF_t + c_F w_t \hat{\bmF}.$
 
 \subsubsection{Optimizing \texorpdfstring{$\bmv$}{v}
  for fixed \texorpdfstring{$\bmF$}{F}}
  Holding $\bmF$ fixed as $\bmF_{t+1}$, the minorizer in \cref{eq:joint_minorizer_Fv} separates in each $v_\ell$ with the following maximizers:
  \begin{align}
      \hat{v}_{\ell} &= \frac{\bar{\alpha}_{t,\ell} - \bar{\rho}_{t,\ell}(\bmF_{t+1})}{\bar{\theta}_{t,\ell}}.
  \end{align}
  For $\ell=g(t)$, we perform the above computation and update $v_{t+1,\ell} = (1- c_v w_t) v_{t,\ell} + c_v w_t \hat{v}_\ell$; otherwise, no update occurs. Since no updates occur to the rows $\bmf_i$ for $i \notin \Omega_t$, we can reuse and downweight the previously computed summands in $\bar{\rho}_{t,\ell}(\bmF_{t+1})$ for $i \notin \Omega_t$ and therefore only compute the summands over $i \in \Omega_t$.
  
 \subsubsection{Memory complexity}
 SHASTA-PCA-2 requires the storage of surrogate parameters $\bbrtheta, \bbralpha, \bbrrho \in \bbR_+^L$ and $\mathcal{O}(dL)$ number of $k\times k$ matrices for the $\bbrR_{t,\ell}(i)$ and $\mathcal{O}(dL)$ number of $k$-length vectors for the $\bbrs_{t,\ell}(i)$. Thus, the total storage scales as $\mathcal{O}(dL(k^2 + k))$.
 
 \subsubsection{Convergence}
 
 In the works \cite{Strohmeier2020OnlineNT,lyu2022convergence}, the authors study stochastic MM for functions that are multi-convex in blocks of variables for the setting of online CP tensor factorization. In their framework, they perform block-coordinate minimization of a single majorizer at each time iteration. They then prove almost sure convergence of the majorizers to a stationary point assuming the expected loss function is continuously differentiable and has Lipschitz gradient, the sequence of non-increasing weights decay at a certain rate, and the data tensors form a Markov chain with a unique stationary distribution.

==> tmlr_instructions.tex <==
\section{Submission of papers to TMLR}

TMLR requires electronic submissions, processed by
\url{https://openreview.net/}. See TMLR's website for more instructions.

If your paper is ultimately accepted, use option {\tt accepted} with the {\tt tmlr} 
package to adjust the format to the camera ready requirements, as follows:
\begin{center}  
  {\tt {\textbackslash}usepackage[accepted]\{tmlr\}}. 
\end{center}
You also need to specify the month and year
by defining variables {\tt month} and {\tt year}, which respectively
should be a 2-digit and 4-digit number. To de-anonymize and remove mentions
to TMLR (for example for posting to preprint servers), use the preprint option,
as in {\tt {\textbackslash}usepackage[preprint]\{tmlr\}}. 

Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to TMLR must be prepared according to the
instructions presented here.

Authors are required to use the TMLR \LaTeX{} style files obtainable at the
TMLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for TMLR and other journal information are available online on
the TMLR website.
The file \verb+tmlr.pdf+ contains these
instructions and illustrates the
various formatting requirements your TMLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+tmlr.sty+ and \verb+tmlr.bst+ (to be used with \LaTeX{}2e). The file
\verb+tmlr.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 6.5~inches wide and
9~inches long. The left margin is 1~inch.
Use 10~point type with a vertical spacing of 11~points. Computer Modern Bright is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in bold and left-aligned.
All pages should start at 1~inch from the top of the page.

Authors' names are
set in boldface. Each name is placed above its corresponding
address and has its corresponding email contact on the same line, in italic 
and right aligned. The lead author's name is to be listed first, and
the co-authors' names are set to follow vertically.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

First level headings are in bold,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in bold,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in bold,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis, using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textbf{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches.\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}. Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Broader Impact Statement}
In this optional section, TMLR encourages authors to discuss possible repercussions of their work,
notably any potential negative impact that a user of this research should be aware of. 
Authors should consult the TMLR Ethics Guidelines available on the TMLR website
for guidance on how to approach this subject.

\subsubsection*{Author Contributions}
If you'd like to, you may include a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors. Only add
this information once your submission is accepted and deanonymized. 

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.
Only add this information once your submission is accepted and deanonymized. 

\bibliography{main}
\bibliographystyle{tmlr}

\appendix
\section{Appendix}
You may include other additional sections here.
